Measuring the False Sense of Security

Recently, several papers have demonstrated how widespread gradient masking is amongst proposed adversarial defenses. Defenses that rely on this phenomenon are considered failed, and can easily be broken. Despite this, there has been little investigation into ways of measuring the phenomenon of gradient masking and enabling comparisons of its extent amongst different networks. In this work, we investigate gradient masking under the lens of its mensurability, departing from the idea that it is a binary phenomenon. We propose and motivate several metrics for it, performing extensive empirical tests on defenses suspected of exhibiting different degrees of gradient masking. These are computationally cheaper than strong attacks, enable comparisons between models, and do not require the large time investment of tailor-made attacks for specific models. Our results reveal metrics that are successful in measuring the extent of gradient masking across different networks

==> figures/grad_mask_plot.tex <==
\begin{figure}
\centering
\begin{tabular}{cc}
  \includegraphics[width=65mm]{figures/plot_along_grad/undefended.png} &   \includegraphics[width=65mm]{figures/plot_along_grad/fgsm model no grad mask.png} \\
(a) Undefended & (b) FGSM $\epsilon = 8/255$ \\[6pt]
 \includegraphics[width=65mm]{figures/plot_along_grad/fgsm_small.png} &   \includegraphics[width=65mm]{figures/plot_along_grad/fgsm.png} \\
(c) FGSM $\epsilon = 8/255$ (CO) & (d) FGSM $\epsilon = 16/255$ \\[6pt]
\includegraphics[width=65mm]{figures/plot_along_grad/step_ll_small.png} &   \includegraphics[width=65mm]{figures/plot_along_grad/step_ll.png} \\
(e) Step-ll $\epsilon = 8/255$ & (f) Step-ll $\epsilon = 16/255$ \\[6pt]
\includegraphics[width=65mm]{figures/plot_along_grad/grad_reg_01.png} &   \includegraphics[width=65mm]{figures/plot_along_grad/grad_reg_05.png} \\
(g) Jacobian Regularization 0.1 & (h) Jacobian Regularization 0.5 \\[6pt]
\includegraphics[width=65mm]{figures/plot_along_grad/grad_reg_1.png} &   \includegraphics[width=65mm]{figures/plot_along_grad/cure.png} \\
(i) Jacobian Regularization 1 & (j) CURE \\[6pt]
\multicolumn{2}{c}{\includegraphics[width=65mm]{figures/plot_along_grad/lipschitz.png} }\\
\multicolumn{2}{c}{(k) Gradient Clipping}
\end{tabular}
\caption{Value of loss along the gradient direction at varying values of $\epsilon$. The mean value for each $\epsilon$ is shown in red, bounded by one standard deviation. Samples from random data points are shown in pale blue. On the left are the results for the training set, and on the right for the testing set. The solid green line shows the mean value of the location of the decision boundary, with pale green lines showing one standard deviation in each direction}
\label{plotAlongGrad}
\end{figure}

==> figures/grad_mask_plot_wide.tex <==
\begin{figure}
\centering
\begin{tabular}{ccc}
  \includegraphics[width=55mm]{figures/plot_along_grad/undefended.png} &   \includegraphics[width=55mm]{figures/plot_along_grad/fgsm model no grad mask.png} &
  \includegraphics[width=55mm]{figures/plot_along_grad/fgsm_small.png}
  \\
(a) Undefended & (b) FGSM $\epsilon = 8/255$ & (c) FGSM $\epsilon = 8/255$\\[6pt]
  \includegraphics[width=55mm]{figures/plot_along_grad/fgsm.png} &
  \includegraphics[width=55mm]{figures/plot_along_grad/step_ll_small.png} &   \includegraphics[width=55mm]{figures/plot_along_grad/step_ll.png}\\
(d) FGSM $\epsilon = 16/255$ &
(e) Step-ll $\epsilon = 8/255$ & (f) Step-ll $\epsilon = 16/255$ \\[6pt]
\includegraphics[width=55mm]{figures/plot_along_grad/grad_reg_01.png} &   \includegraphics[width=55mm]{figures/plot_along_grad/grad_reg_05.png} &
\includegraphics[width=55mm]{figures/plot_along_grad/grad_reg_1.png}\\
(g) Jacobian Regularization 0.1 & (h) Jacobian Regularization 0.5 &
(i) Jacobian Regularization 1 \\[6pt]
 \includegraphics[width=55mm]{figures/plot_along_grad/cure.png} & \includegraphics[width=55mm]{figures/plot_along_grad/lipschitz.png}\\
(j) CURE & (k) Lipschitz \\[6pt]
\end{tabular}
\caption{Value of loss along the gradient direction at varying values of $\epsilon$. The mean value for each $\epsilon$ is shown in red, bounded by one standard deviation. Samples from random data points are shown in pale blue. On the left are the results for the training set, and on the right for the testing set. The solid green line shows the mean value for of the location of the decision boundary, with pale green lines showing one standard deviation in each direction}
\label{plotAlongGrad}
\end{figure}

==> figures/scatter.tex <==
\begin{figure}[ht]
\centering
\begin{tabular}{cc}
  \includegraphics[width=120mm]{figures/Gradient Norm_AA_Train.png} \\ \includegraphics[width=120mm]{figures/FGSM PGD Cosine Similarity eps 006_AA_Test.png} \\
  \includegraphics[width=120mm]{figures/PGD collinearity_AA_Test.png}
\end{tabular}
\caption{Scatter plots for reported - Autoattack accuracy vs metric score for 3 chosen metrics. Shown for training data for the Gradient Norm metric and testing data for the remaining two. The blue line shows the metric value for a normally trained WideResNet-28. A clear correlation between the metric value and how inaccurate the robustness estimate was can be clearly observed.}
\label{scatter}
\end{figure}

==> sections/Discussion.tex <==
\section{Discussion}
One may find it strange that for some of these metrics an undefended model scores very similarly to the Step-ll defense, raising the possibility of false positives. However, the consideration of gradient masking for a model only makes sense once the model has shown good adversarial accuracy against at least single step attacks. If this is not the case then the gradients are clearly not masked. Addressing this issue should be as simple as ensuring that these metrics are analysed together with adversarial accuracy for each network using single step and iterative attacks. 

A more serious limitation is the need for a benchmark such as PGD for these results. This is an issue as these metrics cannot be considered architecture agnostic. Thus, for each neural network architecture being considered, a reliable benchmark from a robust model must first be established in order to extract any meaning from metrics on the target model.

Another concern is that some of these metrics may not apply universally. Indeed, they are not based on hard theoretical evidence, but rather intuition and empirical results. For instance, while models that use gradient masking as a strategy will be less linearizable, a priori, a model that is not linearizable is not necessarily not robust. Metrics like the linearization error or PGD collinearity may indicate that a model is gradient masking in this case. However, research has shown that model robustness can be associated with models that are more linear around the data points. Our own results across these metrics support the idea that highly non-linear loss surfaces are in general not desirable or usual in a neural network.

An interesting group of results are those for the Jacobian regularization models. While our benchmarks did not recognize signs of gradient masking, it is nonetheless interesting that this defense performed similarly to gradient masked models in some metrics. While it could be a testament to the ineffectiveness of some metrics, it could also signal that these models may rely, to some extent, on gradient masking.

Finally, we can address the disappointing results of the robustness information metric. Interestingly, this metric clearly identifies the Step-ll defense with $\epsilon = 16/255$ as gradient masking. This defense had been the most elusive for other metrics to clearly identify as such. However, PGD models actually achieve a lower score than the problematic FGSM models, which are the most evident cases of gradient masking, removing some credibility from this metric.

While we do not believe the intuition behind the metric to be fundamentally flawed, there are some possible reasons for its relative failure. First of all, the metric completely relies on DeepFool. It is possible that the final result is highly dependent on how effective DeepFool is on each separate network. The second consideration is that, in models that are more robust, such as those trained using PGD, we would expect the decision boundary to be further away from the data point. Thus, it may be somewhat unfair that we are comparing the direction given at a boundary which is further away to be as reliable as that given at a boundary which is much closer to the data point.


==> sections/Related.tex <==
However, as shown not only in the original paper, but also later throughout the literature \citep{papernot2016science, tramerAdaptive, obfuscated}, defenses that produce networks where gradients are masked fail to truly improve robustness. 

Since the initial definition of gradient masking by \citep{papernotPractical}, many works have explored the topic.\citet{ensemble} shows that "adversarial training with single-step methods admits a degenerate global minimum, wherein the model’s loss can not be reliably approximated by a linear function", offering some explanation for the phenomenon of gradient masking. \citet{obfuscated} focus on cases of defenses proposed by the research community whose design masks gradients, so called "obfuscated gradients", and effectively break them. \citet{tramerAdaptive} demonstrates that defenses that rely on gradient masking are often still vulnerable to other attacks, some of which may involve only slight tweaks to the original attack formulation. These are in general considered to be failed defenses. However, the adaptations made to attacks must be specific to each defense, and their design is usually not trivial. When evaluating if a network's gradients are being masked, this process is thus too inefficient. We envision a metric for gradient masking, akin to the validation accuracy for overfitting, that could facilitate this evaluation. However, in general, how gradient masking occurs is not well understood, and even a rigorous definition of what exactly it comprises has not been established. 



%related
These include:

\begin{itemize}
    \item Black box attacks outperform white box attacks
    \item Unbounded attacks do not reach $100\%$ fooling rate
    \item Increasing the distortion bound does not decrease accuracy
\end{itemize}


%later section
Black box attacks are those that only have access to the output of the model, and therefore do not make use of any of its gradients (e.g. SPSA, model transfer attacks). White box attacks have access to the model and its gradients. Black box attacks are a strict subset of white box attacks, and should not outperform them \cite{obfuscated}. Additionally, \citet{ensemble} measures the difference between the loss value achieved by a single step attack and an iterative attack. Models where this difference is large are less amenable to linearization and, as such, their gradients may be masked. They further briefly mention comparisons between the perturbation vectors returned by single and iterative attacks as measures of a model’s amenability to linearization.

\subsection{Limitations and Project Goal}
While the behaviours described in \citep{obfuscated} can serve as a checklist to confirm whether the network under consideration suffers from gradient masking, they are quite crude tools for the task. Looking for certain characteristic behaviours in a checklist manner is inherently opaque, not providing insights into what is happening to the loss surface in gradient masked networks. Furthermore, these tests are mostly binary in output, disregarding the extent to which gradient masking takes place. This leads to a further problem in establishing insightful comparisons between models and evaluating potential proposed improvements to defenses with regard to gradient masking. These methods are also very time consuming, with black box attacks in particular tending to require excessive computational resources and being very sensitive to the chosen hyperparameters. 

%related
As for the measures mentioned by \citet{ensemble}, sufficient empirical evidence and results on different defenses are lacking to establish their usefulness beyond interesting figures.


==> tables/Test_aggregated_metrics_table.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrr}
\toprule
                                index & Clean Accuracy & \multicolumn{2}{l}{FGSM Accuracy} & \multicolumn{3}{l}{PGD Accuracy} & \multicolumn{2}{l}{SPSA Accuracy} & Gradient Norm & \multicolumn{2}{l}{FGSM PGD Cosine Similarity} & \multicolumn{2}{l}{Linearization Error} & PGD Collinearity & Gradient Information \\
                                      &              - &         8/255 & 16/255 &        8/255 & 16/255 & Unbounded &         8/255 & 16/255 &             - &                      8/255 &  16/255 &               8/255 &    16/255 &                - &                    - \\
\midrule
                  ResNet-18 20 epochs &           81.5 &           3.0 &    2.5 &          0.0 &    0.0 &       0.0 &          12.0 &   10.0 &        0.2544 &                     0.2905 &  0.1750 &              5.3513 &   14.0136 &           0.1694 &               0.7821 \\
                     Normal ResNet-18 &           97.5 &          43.0 &   24.5 &          0.0 &    0.0 &       0.0 &           0.0 &    0.0 &        0.0680 &                     0.0641 &  0.0297 &              3.8535 &   30.1789 &           0.0382 &               0.3359 \\
              Step-ll \textbackslash epsilon: 8/255 &           74.0 &          31.5 &   13.5 &         23.5 &    4.5 &       0.0 &          41.0 &   19.0 &        0.0524 &                     0.6404 &  0.4973 &              1.0557 &    1.4191 &           0.5056 &               0.8324 \\
             Step-ll \textbackslash epsilon: 16/255 &           70.5 &          57.0 &   53.5 &          3.0 &    0.5 &       0.0 &           8.0 &    3.0 &        0.2392 &                     0.2214 &  0.1255 &              2.6540 &    4.2211 &           0.1959 &               0.5433 \\
                 FGSM \textbackslash epsilon: 8/255 &           67.0 &          33.5 &   17.0 &         27.5 &    7.0 &       0.0 &          40.0 &   22.0 &        0.0236 &                     0.6958 &  0.5505 &              0.2964 &    0.7265 &           0.5583 &               0.8390 \\
            FGSM \textbackslash epsilon: 8/255 (CO) &           78.0 &          73.0 &   57.5 &          0.0 &    0.0 &       0.0 &           2.0 &    3.0 &        0.3972 &                     0.0669 &  0.0466 &              3.3727 &  148.5161 &           0.0642 &               0.5629 \\
                FGSM \textbackslash epsilon: 16/255 &           71.0 &          77.0 &   88.5 &          0.0 &    0.0 &       0.0 &           1.0 &    1.0 &        0.7424 &                     0.0658 &  0.0274 &             11.2783 &   12.3902 &           0.0776 &               0.7944 \\
                  PGD \textbackslash epsilon: 8/255 &           66.0 &          35.0 &   17.0 &         29.5 &    8.0 &       0.0 &          39.0 &   25.0 &        0.0204 &                     0.7190 &  0.5761 &              0.4278 &    0.5711 &           0.5858 &               0.8512 \\
                 PGD \textbackslash epsilon: 16/255 &           53.5 &          39.0 &   27.0 &         38.0 &   23.0 &       0.0 &          36.0 &   30.0 &        0.0083 &                     0.7907 &  0.6794 &              0.2232 &    0.7346 &           0.6797 &               0.8078 \\
 Jacobian Regularization \textbackslash lambda: 0.1 &           77.5 &          12.0 &    2.5 &          4.5 &    0.0 &       0.0 &          18.0 &    5.0 &        0.0435 &                     0.5827 &  0.4097 &              1.1094 &    4.1042 &           0.4325 &               0.8712 \\
 Jacobian Regularization \textbackslash lambda: 0.5 &           71.0 &          15.0 &    1.5 &          9.0 &    0.5 &       0.0 &          19.0 &    6.0 &        0.0324 &                     0.6447 &  0.4603 &              0.5211 &    4.1131 &           0.5048 &               0.9088 \\
   Jacobian Regularization \textbackslash lambda: 1 &           63.5 &          18.5 &    3.5 &         13.0 &    1.0 &       0.0 &          22.0 &   11.0 &        0.0246 &                     0.6739 &  0.4985 &              0.4942 &    2.4398 &           0.5695 &               0.9074 \\
                            Lipschitz &           93.0 &          54.0 &   39.0 &         11.5 &    4.0 &       0.0 &          41.0 &   29.0 &        0.1014 &                     0.1207 &  0.0504 &              4.6295 &   18.4991 &           0.0572 &               0.1354 \\
                                 CURE &           77.5 &          40.5 &   15.5 &         35.5 &    8.0 &       0.0 &          48.0 &   27.0 &        0.0115 &                     0.7713 &  0.6288 &              0.3390 &    0.4483 &           0.6674 &               0.9045 \\
            Adversarial Interpolation &           91.5 &          76.0 &   74.5 &         73.5 &   70.0 &       4.0 &          73.0 &   73.0 &        0.0222 &                     0.4473 &  0.2935 &              2.9747 &    9.3566 &           0.2951 &               0.1579 \\
                      Feature Scatter &           87.0 &          71.5 &   71.0 &         67.5 &   61.5 &       0.0 &          67.0 &   66.0 &        0.0207 &                     0.4814 &  0.2980 &              2.0111 &    8.0076 &           0.3090 &               0.2075 \\
                             Standard &           93.0 &          28.0 &   18.5 &          0.0 &    0.0 &       0.0 &           0.0 &    0.0 &        0.2058 &                     0.0725 &  0.0369 &              4.0258 &   60.7705 &           0.0457 &               0.4470 \\
      Gowal2020Uncovering\_28\_10\_extra &           88.0 &          68.0 &   51.5 &         65.0 &   37.0 &       0.0 &          70.0 &   55.0 &        0.0085 &                     0.7515 &  0.5623 &              0.0906 &    0.2208 &           0.6496 &               0.5349 \\
              Wu2020Adversarial\_extra &           88.0 &          64.0 &   47.5 &         60.5 &   34.5 &       0.0 &          63.0 &   51.0 &        0.0094 &                     0.7168 &  0.5352 &              0.0892 &    0.2388 &           0.6081 &               0.5969 \\
                  Carmon2019Unlabeled &           88.0 &          66.5 &   49.0 &         59.0 &   33.0 &       0.0 &          65.0 &   53.0 &        0.0104 &                     0.6755 &  0.4837 &              0.0924 &    0.2386 &           0.5578 &               0.5052 \\
                    Wang2020Improving &           87.5 &          67.0 &   49.5 &         62.0 &   34.0 &       0.0 &          67.0 &   55.0 &        0.0102 &                     0.6514 &  0.4613 &              0.1340 &    0.3150 &           0.5292 &               0.5530 \\
                    Zhang2020Geometry &           90.0 &          66.5 &   44.0 &         66.5 &   38.5 &       0.0 &          70.0 &   55.0 &        0.0104 &                     0.6755 &  0.4947 &              0.1258 &    0.3046 &           0.5626 &               0.6638 \\
                         Wong2020Fast &           83.5 &          55.0 &   31.0 &         49.5 &   15.5 &       0.0 &          60.0 &   36.0 &        0.0110 &                     0.6864 &  0.4883 &              0.3894 &    0.4619 &           0.5593 &               0.7331 \\
                   Hendrycks2019Using &           84.5 &          61.0 &   43.5 &         56.0 &   25.5 &       0.0 &          66.0 &   50.0 &        0.0102 &                     0.7162 &  0.5285 &              0.1091 &    0.2439 &           0.5769 &               0.6360 \\
                      Sehwag2020Hydra &           88.5 &          64.5 &   48.5 &         58.5 &   31.0 &       0.0 &          67.0 &   47.0 &        0.0104 &                     0.7010 &  0.5240 &              0.6919 &    1.7393 &           0.5842 &               0.5416 \\
\bottomrule
\end{tabular}


==> tables/Test_relative_metrics_table.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
                                index & Gradient Norm & \multicolumn{2}{l}{FGSM PGD Cosine Similarity} & \multicolumn{2}{l}{Linearization Error} & PGD Collinearity & Gradient Information \\
                                      &             - &                      8/255 & 16/255 &               8/255 & 16/255 &                - &                    - \\
\midrule
                  ResNet-18 20 epochs &          3065 &                         36 &     25 &                2397 &   1907 &               24 &                   96 \\
                     Normal ResNet-18 &           819 &                          8 &      4 &                1726 &   4108 &                5 &                   41 \\
              Step-ll \textbackslash epsilon: 8/255 &           631 &                         80 &     73 &                 472 &    193 &               74 &                  103 \\
             Step-ll \textbackslash epsilon: 16/255 &          2881 &                         28 &     18 &                1189 &    574 &               28 &                   67 \\
                 FGSM \textbackslash epsilon: 8/255 &           284 &                         87 &     81 &                 132 &     98 &               82 &                  103 \\
            FGSM \textbackslash epsilon: 8/255 (CO) &          4785 &                          8 &      6 &                1511 &  20217 &                9 &                   69 \\
                FGSM \textbackslash epsilon: 16/255 &          8944 &                          8 &      4 &                5053 &   1686 &               11 &                   98 \\
                  PGD \textbackslash epsilon: 8/255 &           245 &                         90 &     84 &                 191 &     77 &               86 &                  105 \\
                 PGD \textbackslash epsilon: 16/255 &           100 &                        100 &    100 &                 100 &    100 &              100 &                  100 \\
 Jacobian Regularization \textbackslash lambda: 0.1 &           524 &                         73 &     60 &                 497 &    558 &               63 &                  107 \\
 Jacobian Regularization \textbackslash lambda: 0.5 &           390 &                         81 &     67 &                 233 &    559 &               74 &                  112 \\
   Jacobian Regularization \textbackslash lambda: 1 &           296 &                         85 &     73 &                 221 &    332 &               83 &                  112 \\
                            Lipschitz &          1221 &                         15 &      7 &                2074 &   2518 &                8 &                   16 \\
                                 CURE &           138 &                         97 &     92 &                 151 &     61 &               98 &                  111 \\
            Adversarial Interpolation &           267 &                         56 &     43 &                1332 &   1273 &               43 &                   19 \\
                      Feature Scatter &           249 &                         60 &     43 &                 901 &   1090 &               45 &                   25 \\
                             Standard &          2479 &                          9 &      5 &                1803 &   8272 &                6 &                   55 \\
      Gowal2020Uncovering\_28\_10\_extra &           102 &                         95 &     82 &                  40 &     30 &               95 &                   66 \\
              Wu2020Adversarial\_extra &           113 &                         90 &     78 &                  39 &     32 &               89 &                   73 \\
                  Carmon2019Unlabeled &           125 &                         85 &     71 &                  41 &     32 &               82 &                   62 \\
                    Wang2020Improving &           122 &                         82 &     67 &                  60 &     42 &               77 &                   68 \\
                    Zhang2020Geometry &           125 &                         85 &     72 &                  56 &     41 &               82 &                   82 \\
                         Wong2020Fast &           132 &                         86 &     71 &                 174 &     62 &               82 &                   90 \\
                   Hendrycks2019Using &           122 &                         90 &     77 &                  48 &     33 &               84 &                   78 \\
                      Sehwag2020Hydra &           125 &                         88 &     77 &                 309 &    236 &               85 &                   67 \\
\bottomrule
\end{tabular}


==> tables/Train_aggregated_metrics_table.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrr}
\toprule
                                index & Clean Accuracy & \multicolumn{2}{l}{FGSM Accuracy} & \multicolumn{3}{l}{PGD Accuracy} & \multicolumn{2}{l}{SPSA Accuracy} & Gradient Norm & \multicolumn{2}{l}{FGSM PGD Cosine Similarity} & \multicolumn{2}{l}{Linearization Error} & PGD Collinearity & Gradient Information \\
                                      &              - &         8/255 & 16/255 &        8/255 & 16/255 & Unbounded &         8/255 & 16/255 &             - &                      8/255 &  16/255 &               8/255 &   16/255 &                - &                    - \\
\midrule
                  ResNet-18 20 epochs &          100.0 &           6.5 &    4.5 &          0.0 &    0.0 &       0.0 &           6.0 &    7.0 &        0.0001 &                     0.2894 &  0.1641 &              0.8206 &   3.6068 &           0.1734 &               0.6891 \\
                     Normal ResNet-18 &          100.0 &          44.5 &   20.0 &          0.0 &    0.0 &       0.0 &           1.0 &    0.0 &        0.0007 &                     0.0629 &  0.0279 &              1.7604 &  16.6680 &           0.0372 &               0.2084 \\
              Step-ll \textbackslash epsilon: 8/255 &           99.5 &          70.0 &   18.0 &         44.5 &    3.5 &       0.0 &          86.0 &   32.0 &        0.0006 &                     0.6181 &  0.4757 &              0.0973 &   0.1991 &           0.4970 &               0.7242 \\
             Step-ll \textbackslash epsilon: 16/255 &           97.5 &          98.5 &   96.5 &          2.5 &    0.5 &       0.0 &          11.0 &    2.0 &        0.0240 &                     0.2243 &  0.1199 &              0.4326 &   0.8501 &           0.1935 &               0.3091 \\
                 FGSM \textbackslash epsilon: 8/255 &           94.5 &          77.5 &   40.5 &         69.5 &   12.0 &       0.0 &          82.0 &   62.0 &        0.0039 &                     0.6875 &  0.5303 &              0.0723 &   0.1547 &           0.5661 &               0.7278 \\
            FGSM \textbackslash epsilon: 8/255 (CO) &           95.0 &          96.5 &   82.5 &          0.0 &    0.0 &       0.0 &           7.0 &    7.0 &        0.1124 &                     0.0706 &  0.0429 &              1.0983 &   7.1962 &           0.0664 &               0.4743 \\
                FGSM \textbackslash epsilon: 16/255 &           79.5 &          89.0 &   98.0 &          0.0 &    0.0 &       0.0 &           1.0 &    1.0 &        0.5189 &                     0.0665 &  0.0286 &              2.3537 &  12.0186 &           0.0785 &               0.7911 \\
                  PGD \textbackslash epsilon: 8/255 &           91.5 &          75.5 &   43.5 &         67.0 &   22.0 &       0.0 &          81.0 &   54.0 &        0.0049 &                     0.7179 &  0.5632 &              0.0708 &   0.1525 &           0.5956 &               0.7450 \\
                 PGD \textbackslash epsilon: 16/255 &           59.0 &          46.0 &   36.5 &         45.0 &   29.0 &       0.0 &          43.0 &   34.0 &        0.0057 &                     0.7843 &  0.6734 &              0.0795 &   0.2743 &           0.6878 &               0.7739 \\
 Jacobian Regularization \textbackslash lambda: 0.1 &           96.5 &          11.5 &    1.0 &          5.0 &    0.0 &       0.0 &          18.0 &    6.0 &        0.0134 &                     0.5981 &  0.4158 &              0.2254 &   0.6395 &           0.4389 &               0.8639 \\
 Jacobian Regularization \textbackslash lambda: 0.5 &           83.0 &          15.5 &    2.0 &          8.0 &    0.0 &       0.0 &          14.0 &    4.0 &        0.0223 &                     0.6494 &  0.4700 &              0.1889 &   0.4389 &           0.5090 &               0.8978 \\
   Jacobian Regularization \textbackslash lambda: 1 &           70.5 &          21.0 &    4.5 &         14.0 &    0.5 &       0.0 &          20.0 &    7.0 &        0.0234 &                     0.6787 &  0.4945 &              0.2842 &   1.0912 &           0.5700 &               0.9047 \\
                            Lipschitz &          100.0 &          62.5 &   50.0 &         15.5 &    3.0 &       0.0 &          38.0 &   29.0 &        0.0001 &                     0.1093 &  0.0416 &              1.4494 &   8.7681 &           0.0565 &               0.0187 \\
                                 CURE &           92.0 &          48.5 &   17.5 &         43.5 &   10.5 &       0.0 &          58.0 &   29.0 &        0.0080 &                     0.7727 &  0.6267 &              0.0794 &   0.1703 &           0.6739 &               0.8902 \\
            Adversarial Interpolation &          100.0 &         100.0 &  100.0 &         99.0 &   97.0 &       1.5 &         100.0 &   99.0 &        0.0015 &                     0.5167 &  0.3549 &              0.0136 &   0.0275 &           0.3596 &               0.0063 \\
                      Feature Scatter &           99.5 &          98.5 &   97.0 &         97.5 &   87.5 &       0.5 &          99.0 &   99.0 &        0.0021 &                     0.5320 &  0.3487 &              0.0192 &   0.1383 &           0.3692 &               0.0204 \\
                             Standard &          100.0 &          31.0 &   22.5 &          0.0 &    0.0 &       0.0 &           0.0 &    0.0 &        0.0001 &                     0.0707 &  0.0351 &              2.2751 &  16.2693 &           0.0440 &               0.3417 \\
      Gowal2020Uncovering\_28\_10\_extra &           95.0 &          82.0 &   72.0 &         79.0 &   52.0 &       0.0 &          84.0 &   75.0 &        0.0050 &                     0.7667 &  0.5714 &              0.0513 &   0.1289 &           0.6624 &               0.4558 \\
              Wu2020Adversarial\_extra &           94.0 &          83.5 &   66.0 &         80.5 &   46.5 &       0.0 &          86.0 &   73.0 &        0.0053 &                     0.7201 &  0.5330 &              0.0553 &   0.1427 &           0.6168 &               0.5100 \\
                  Carmon2019Unlabeled &           98.0 &          85.5 &   75.0 &         82.0 &   44.5 &       0.0 &          89.0 &   78.0 &        0.0045 &                     0.6932 &  0.4936 &              0.0499 &   0.1219 &           0.5780 &               0.3930 \\
                    Wang2020Improving &           90.5 &          76.0 &   61.5 &         72.0 &   39.0 &       0.0 &          80.0 &   67.0 &        0.0073 &                     0.6594 &  0.4659 &              0.1077 &   0.2410 &           0.5386 &               0.4915 \\
                    Zhang2020Geometry &           94.5 &          83.0 &   66.0 &         80.0 &   52.0 &       0.0 &          84.0 &   77.0 &        0.0065 &                     0.6826 &  0.4944 &              0.0975 &   0.2377 &           0.5715 &               0.6073 \\
                         Wong2020Fast &           86.0 &          59.5 &   37.5 &         53.0 &   15.0 &       0.0 &          67.0 &   40.0 &        0.0082 &                     0.6851 &  0.4833 &              0.0971 &   0.2272 &           0.5589 &               0.7162 \\
                   Hendrycks2019Using &           87.0 &          66.0 &   43.5 &         62.5 &   26.5 &       0.0 &          67.0 &   48.0 &        0.0099 &                     0.7181 &  0.5304 &              0.1213 &   0.2994 &           0.5886 &               0.6379 \\
                      Sehwag2020Hydra &           94.5 &          82.5 &   66.5 &         79.0 &   40.0 &       0.0 &          80.0 &   72.0 &        0.0053 &                     0.7144 &  0.5233 &              0.2054 &   1.2457 &           0.5963 &               0.4668 \\
\bottomrule
\end{tabular}


==> tables/Train_relative_metrics_table.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
                                index & Gradient Norm & \multicolumn{2}{l}{FGSM PGD Cosine Similarity} & \multicolumn{2}{l}{Linearization Error} & PGD Collinearity & Gradient Information \\
                                      &             - &                      8/255 & 16/255 &               8/255 & 16/255 &                - &                    - \\
\midrule
                  ResNet-18 20 epochs &             1 &                         36 &     24 &                1032 &   1314 &               25 &                   89 \\
                     Normal ResNet-18 &            12 &                          8 &      4 &                2214 &   6076 &                5 &                   26 \\
              Step-ll \textbackslash epsilon: 8/255 &            10 &                         78 &     70 &                 122 &     72 &               72 &                   93 \\
             Step-ll \textbackslash epsilon: 16/255 &           421 &                         28 &     17 &                 544 &    309 &               28 &                   39 \\
                 FGSM \textbackslash epsilon: 8/255 &            68 &                         87 &     78 &                  90 &     56 &               82 &                   94 \\
            FGSM \textbackslash epsilon: 8/255 (CO) &          1971 &                          9 &      6 &                1381 &   2623 &                9 &                   61 \\
                FGSM \textbackslash epsilon: 16/255 &          9103 &                          8 &      4 &                2960 &   4381 &               11 &                  102 \\
                  PGD \textbackslash epsilon: 8/255 &            85 &                         91 &     83 &                  89 &     55 &               86 &                   96 \\
                 PGD \textbackslash epsilon: 16/255 &           100 &                        100 &    100 &                 100 &    100 &              100 &                  100 \\
 Jacobian Regularization \textbackslash lambda: 0.1 &           235 &                         76 &     61 &                 283 &    233 &               63 &                  111 \\
 Jacobian Regularization \textbackslash lambda: 0.5 &           391 &                         82 &     69 &                 237 &    160 &               74 &                  116 \\
   Jacobian Regularization \textbackslash lambda: 1 &           410 &                         86 &     73 &                 357 &    397 &               82 &                  116 \\
                            Lipschitz &             1 &                         13 &      6 &                1823 &   3196 &                8 &                    2 \\
                                 CURE &           140 &                         98 &     93 &                  99 &     62 &               97 &                  115 \\
            Adversarial Interpolation &            26 &                         65 &     52 &                  17 &     10 &               52 &                    0 \\
                      Feature Scatter &            36 &                         67 &     51 &                  24 &     50 &               53 &                    2 \\
                             Standard &             1 &                          9 &      5 &                2861 &   5931 &                6 &                   44 \\
      Gowal2020Uncovering\_28\_10\_extra &            87 &                         97 &     84 &                  64 &     46 &               96 &                   58 \\
              Wu2020Adversarial\_extra &            92 &                         91 &     79 &                  69 &     52 &               89 &                   65 \\
                  Carmon2019Unlabeled &            78 &                         88 &     73 &                  62 &     44 &               84 &                   50 \\
                    Wang2020Improving &           128 &                         84 &     69 &                 135 &     87 &               78 &                   63 \\
                    Zhang2020Geometry &           114 &                         87 &     73 &                 122 &     86 &               83 &                   78 \\
                         Wong2020Fast &           143 &                         87 &     71 &                 122 &     82 &               81 &                   92 \\
                   Hendrycks2019Using &           173 &                         91 &     78 &                 152 &    109 &               85 &                   82 \\
                      Sehwag2020Hydra &            92 &                         91 &     77 &                 258 &    454 &               86 &                   60 \\
\bottomrule
\end{tabular}

